DiffusionPID: Interpreting Diffusion via Partial Information Decomposition

Text-to-image diffusion models have made significant progress in generating naturalistic images from textual inputs, and demonstrate the capacity to learn and represent complex visual-semantic relationships. While these diffusion models have achieved remarkable success, the underlying mechanisms driving their performance are not yet fully accounted for, with many unanswered questions surrounding what they learn, how they represent visual-semantic relationships, and why they sometimes fail to generalize. Our work presents Diffusion Partial Information Decomposition (DiffusionPID), a novel technique that applies information-theoretic principles to decompose the input text prompt into its elementary components, enabling a detailed examination of how individual tokens and their interactions shape the generated image. We introduce a formal approach to analyze the uniqueness, redundancy, and synergy terms by applying PID to the denoising model at both the image and pixel level. This approach enables us to characterize how individual tokens and their interactions affect the model output. We first present a fine-grained analysis of characteristics utilized by the model to uniquely localize specific concepts, we then apply our approach in bias analysis and show it can recover gender and ethnicity biases. Finally, we use our method to visually characterize word ambiguity and similarity from the model's perspective and illustrate the efficacy of our method for prompt intervention. Our results show that PID is a potent tool for evaluating and diagnosing text-to-image diffusion models.

==> sections/02_Intro_backup.tex <==


% Diffusion models have revolutionized the field of text-to-image generation, achieving remarkable results in creating high-fidelity images conditioned on textual descriptions. With their rising adoption in many different domains, it raises concerns over the explainability and safety of these models. For a long time, they have been treated as black boxes with little understanding of how they operate, where they fail, and why they produce the outputs they do. Thus, it becomes crucial to understand the inner workings of such models in depth. This will help build trust in them through increased transparency and can also be used to appropriately account for their limitations and improve upon them. 

Often when working with such generative models, we observe that the generated output is not exactly aligned with our expectations. This can  often happen because of a lack of relation, attribution, and/or compositional understanding of generative models like diffusion models.\cite{rombach2022high}. But often modifying the prompt to a form that might not even seem natural to most humans, gets the original intended output from the model. This gap in the interpretation of humans and diffusion models about different concepts and their interaction is often attempted to be solved by either trial-error or posthoc explanations.  This could also lead to solutions derived from spurious correlations observed \cite{nam2022breaking}. Hence, for a given instance of a generative model like diffusion, their concept understanding, or relations might not match exactly with that of humans. Given 2 terms/concepts, one of them might be redundant to us as humans, but it might not be redundant for the model \rbz{GIVE EXAMPLE?" will need ex to explain disparity both ways} . The terms can get something unique out of the model or even have some synergistic effect. Thus while working with generative models, to get the most of a given model, knowing the understanding of the model of our world and different concepts becomes very important.

Although extensive work has been done to shed light on these models' conceptual understanding and their failure cases, they do so at a very broad level and do not explore the contribution and interaction of the individual terms in the conditioning prompts and their effect on the corresponding image from the models' perspective. Thus, we leverage the concepts of Mutual Information (MI) and Partial Information Decomposition (PID) from information theory to gain insights along this direction. 

\textbf{Mutual Information (MI)} is a measure that estimates the amount of information obtained for an output variable from an input variable passed through a function. It basically measures how much knowing one variable reduces the uncertainty about the other variable In deep learning, where understanding the dependencies and mapping between input features and target variables is vital, MI serves as a powerful tool to quantify these dependencies accurately. 

%\sheenu{which says that the mutual information measures the amount of information that one random variable contains about another random variable. The intuition behind this is that it measures how much knowing one variable reduces the uncertainty about the other variable. Higher mutual information indicates a stronger dependence between the variables}

\textbf{Partial Information Decomposition (PID)} as per \cite{finn2018pointwise} shows that 2 variables $X_1$ and $X_2$ can contribute to information of a target variable Y, in 4 possible ways, where $X_1$ can provide information about x independently/uniquely, $X_2$ too can provide information about Y independently/uniquely, both $X_1$ \& $X_2$ contribute individually but redundantly (i.e. the same contribution from both) and  $X_1$ \& $X_2$ contribute synergistically (which wouldn't have been possible if either of them couldn't do individually). \cite{finn2018pointwise} also state that Mutual information can be derived from first principles as fundamentally pointwise quantities, where they measure information content of individual events. The overall (average) mutual information can then be calculated by taking the expectation over all events from the relevant variables.  


Thus, based on the widely used definition of Mutual Information proposed by \cite{6773024,delgadoshannon}  and inspired by the MI definition from \cite{kong2023interpretable} and point-wise PID by \cite{finn2018pointwise}, we develop our approach of \textbf{P}artial \textbf{I}nformation \textbf{D}ecomposition\textbf{ (PID)} of Diffusion. Our method decomposes the mutual information between 2 terms in the input prompt for the corresponding image into the components of redundancy (R), synergy (S), and uniqueness (U).


 % To understand this better we have to take a look at the outputs of a diffusion model \cite{diffusion}, often working with them it is observed that the generated output is not exactly aligned with our expectations. This might happen due to the lack of semantic understanding the diffusion model has for concepts such as attribution and relation awareness. The compositional understanding of all the objects present in the prompts is also not captured by these models. This issue can be mitigated by modifying the prompt, sometimes to such an extent that does not make perfect sense to humans, but correctly generates the image through a diffusion model. This gap in the interpretation of humans and diffusion models about different concepts and their interaction is often attempted to be solved by either trial-error or posthoc explanations. So due to this underlying gap, if given 2 terms or concepts, the redundancy between them might be high for a diffusion model but not for humans. For example:. 

Along with understanding the specific contribution of the inputs to the output from the model's perspective, this decomposition has many uses. By leveraging synergies, we can construct prompts that elicit richer and more coherent responses from the model. By removing redundant information, we can make prompts more concise and efficient, thereby improving the model's ability to focus on the most relevant aspects of the input. Additionally, identifying redundant information can also aid in designing prompts that are more interpretable and easier for users to understand and manipulate. By introducing unique prompts that deviate from typical patterns or conventions, you can encourage the model to explore new directions and generate responses that are more original and imaginative. Leveraging uniqueness can be particularly valuable in scenarios where generating diverse or novel outputs are desired. Thus we develop 3 datasets viz. Gender Bias, Homonym, WordNet Hyponym,  which help us understand the different aspects of diffusion model and help make informed decision on its dependability. 





 



Thus our main contributions are: \begin{enumerate}
  \item  We give a split of Mutual Information into its inherent components of Synergy, Redundancy and Uniqueness.
  \item Analysis of diffusion model and its failure through the use of redundancy and synergy. 
  \item Identify bias in image-generative models.
  \item Use of PID for for prompt intervention and its use in modifying prompts.
\end{enumerate}



% Various tasks like prompt engineering, ...etc. would hugely benefit from insights into the effects of different terms together and independently in generative models. 






% Their ability to create stunning visuals from textual descriptions highlights their remarkable ability to capture complex relationships between language and visual representations. Yet, like many complex machine learning models, they often operate as "black boxes." This lack of transparency limits our ability to understand why diffusion models make specific decisions and how they arrive at their final image creations. An understanding of the intricate relationship between the input prompt within itself and with the generated image remains a challenge. An understanding of what different element contribute at different granulairities in the generation is required to understand the relation between the input prompt and generated image.



% Works like \cite{liang2024quantifying} focus on the information theoretic approach to extract information of redundancy, synergy and uniqueness relating input with the output between modalities in multimodal settings. Most of such works focus on the factors of synergy, redundancy and uniqueness from human's perspective. Although most work aim/try to make models human aligned, they are still not truly aligned (cite some work that show they are not aligned and frame this better!)  Often when exploring or working with such generative models, we observe that often the generated output is not exactly the way we intended it to be. This can be often because of lack of relations, attributions, compositionally, etc. (CITE WORKS that talk about this). But often modifying the prompt to a form which might not seem natural to most humans, often gets the original intended output from the model. This gap in interpretation of humans and diffusion models about different concepts and their interaction is often attempted to be solved by either trial-error or posthoc explanations which can also lead to solutions derived from spurious correlations observed. Hence, for generative models like diffusion, the concept understanding, and relations need not match exactly with that of humans. Given 2 terms/concepts, one of them might be redundant to us as humans, it might not be redundant for the model. The terms can get something unique out of the model or even have some synergistic effect. Thus while working with generative models, to get the most of a given model, knowing the understanding of the model of our world and different concepts becomes very important. Various tasks like prompt engineering, ...etc. would hugely benefit from insights into the effects of different terms together and independently in generative models.

==> sections/03_Related_backup.tex <==
\section{Related Work}

% Works like\cite{daam,liu2023unsupervised,zhao2023unleashing,tian2023diffuse, attend&excite} use attention-based methods to analyze what part of the generation is caused by a given part of input prompt in diffusion models.
% Whereas, works like \cite{liang2024quantifying} focus on the information theoretic approach to extract information of redundancy (R), synergy (S) and uniqueness (U), where they related input with the output but at the modality level in multimodal settings. Most of such works focus on the factors of S, R and U from human's perspective. Although most generative models are aimed to be models that are human aligned, they are still not truly aligned \cite{ngo2022alignment, ji2023ai, klingefjord2024human}
%(cite some work that show they are not aligned and frame this better!)}  

% \textbf{We disentagle the information learned from MI/CMI. }

\myparagraphzerooffset{Interpretability in AI} The advent of technologies like neural networks and CNNs has changed the face of AI and resulted in a paradigm shift where these technologies are being applied to solve every problem in every domain of AI. This raises concerns about the interpretability and explainability of what these models learn and how they operate, which has resulted in a plethora of work that explores this exact problem. For instance, LIME \cite{lime} presents a technique for interpreting individual predictions of any machine learning (ML) model by approximating it locally with an interpretable model, while SHAP \cite{shap} interprets outputs by assigning each feature in the model an importance value based on Shapley values from cooperative game theory.
%TCAV \cite{Kim2017InterpretabilityBF} uses directional derivatives to quantify a model's prediction's sensitivity to an underlying high-level concept. 
CAM \cite{CAM} and Grad-CAM \cite{gradcam} localize image regions a CNN uses to classify a given image, using a weighted sum of intermediate layers' activations. NetDissect \cite{netdissect} does something similar, but at the neuron level, where they analyze the image regions that most excited a given neuron across all the dataset images while GAN Dissection \cite{gandissect} extends this specifically for GANs. MILAN \cite{milan} builds on top of NetDissect to produce descriptions for each neuron. Along similar lines, CLIP-Dissect \cite{Oikarinen2022CLIPDissectAD} makes use of CLIP to identify semantic concepts corresponding to each neuron. 
% N2G \cite{Foote2023NeuronTG} is the equivalent of NetDissect but for LLMs where their method identifies the tokens an LLM's neuron is most responsive to. 
Some works such as ARO \cite{aro}, Winoground \cite{diwan2022winoground}, EQBEN \cite{Wang2023EquivariantSF}, and WHOOPS \cite{BittonGuetta2023BreakingCS} introduce datasets to specifically test the compositional and semantic understanding of Vision-Language models (VLMs) and show that most SOTA models perform poorly on their benchmarks. 
% Similarly, \cite{Wang2023EquivariantSF} introduces the EQBEN benchmark to study the ability of VLMs to distinguish semantically similar concepts. 
\cite{Wang2022InterpretabilityIT} uses circuit probing to break down a model, specifically GPT-2 small, into circuits and neurons that perform specific tasks. Some works have also explored the application of PID in different settings. \cite{ehrlich2023a} uses PID to measure the contribution of each neuron towards a target concept and \cite{Liang2023QuantifyingM} applies PID on generic multimodal datasets and models. MULTIVIZ \cite{Liang2022MultiVizTV} analyzes the behavior of multimodal models, specifically focusing on the unimodal contributions, cross-modal interactions, and multi-modal representations. Overall, a lot of progress has been made in understanding and interpreting ML models. Given the recent explosion of work on diffusion models, we primarily focus on interpreting these models.

\myparagraphzerooffset{Evaluation and Improvement of Text-to-Image (T2I) Models} In recent times, many works have focused on evaluating the performance of diffusion models, identifying failure cases, and utilizing these insights to improve them. \cite{Saharia2022PhotorealisticTD} introduce the DrawBench benchmark to test various aspects of text-to-image models in challenging situations and go on to propose an improved model, Imagegen. One set of works such as \cite{Hu2023TIFAAA, Lin2024EvaluatingTG, Cho2024DSG} use Visual Question Answering (VQA) to evaluate the quality and fidelity of generated images to the input text prompts. Many T2I models have been shown to struggle with attribution-binding and compositional understanding \cite{Conwell2022TestingRU} which is what TFSDG \cite{tfsdg} improves upon. To address such issues, Attend-and-Excite \cite{Chefer2023AttendandExciteAS}, SynGen \cite{rassin2023linguistic}, \cite{Wang2023CompositionalTS}, and \cite{Phung2023GroundedTS} manipulate the cross-attention layers' excitations whereas \cite{liu2022compositional} composes diffusion models together to generate more faithful images. SAGE \cite{Lin2024EvaluatingTG} proposes an adversarial search method to automatically discover undesirable behaviors and failure cases in image generation. HEIM \cite{lee2023holistic} conducts an extensive analysis of numerous T2I models on many different aspects from text-image alignment to reasoning. Thus, we can see that a lot of work has been done in this domain. Our work is broader, with wider applications, as we focus on studying and understanding diffusion models in depth and our analysis inevitably leads us to identify these models' shortcomings, the reasons behind those failures, and insights that can be applied to enhance them.

\myparagraphzerooffset{Interpretability of Diffusion Models} While diffusion models have come a long way, explaining their behavior remains a challenging task. Data attribution \cite{zheng2023intriguing, georgiev2023journey, Dai2023TrainingDA, wang2023evaluating} is a commonly used approach to pin down which training set samples were most responsible for the appearance of a given generated image. Along a similar direction, \cite{Gal2022AnII, chefer2023hidden} decompose the images associated with a particular concept into the implicit semantic concepts the generative model considers to be most similar. Some works \cite{Kwon2022DiffusionMA, li2023self, Haas2023DiscoveringID, NEURIPS2023_4bfcebed, dalva2023noiseclr} have discovered a semantic latent space for diffusion models such that modifications in this space edit attributes of the original
generated images. \cite{Wu2022UncoveringTD, schrodinger} do something similar but in the text embedding space. Recently, there have also been works that try to gain a neuron-level and network-level understanding of these models. For instance, \cite{lee2023diffusion} divides the latent vector into multiple groups of elements and designs different noise schedules for each group so that each group controls only certain elements of data, explicitly giving interpretable meaning. Similarly, Cones \cite{Liu2023ConesCN} identifies a cluster of neurons corresponding to a given concept using gradient statistics. \cite{schrodinger, double} inspired us to investigate the generative ability of diffusion models on prompts containing homonyms (words with multiple meanings) as these works have shown that diffusion models struggle in such cases. \cite{Luccioni2023StableBE, Orgad2023EditingIA} demonstrated the presence of ethnic, gender, and semantic biases in these models which encouraged us to dive deeper into these using our own method. A recent popular work, DAAM \cite{daam}, analyzes the cross-attention layers of these models to produce attribution maps for tokens from the input prompt. However, these maps are generally very noisy and broad. Also, the maps offer limited information when the model fails to generate a given object.  \cite{kong2023interpretable} introduced a method to compute the mutual information (MI) and conditional mutual information (CMI) between the input text prompt and each generated pixel. While this work proves to be better and more insightful than DAAM in certain cases, it still only provides broad insights into what and how information is used by the model. Thus, we further expand on their work to gain a fine-grained comprehension by further decomposing the MI metric using partial information decomposition (PID).

==> sections/98_Checklist.tex <==

\newpage
\section*{NeurIPS Paper Checklist}

%%% BEGIN INSTRUCTIONS %%%


%%% END INSTRUCTIONS %%%


\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Sections 3 and 4
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A No or NA answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Section 5 has limitations mentioned
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper has no limitation while the answer No means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate "Limitations" section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory Assumptions and Proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Section 3 outlines various theoretical concepts with the required proofs and detailed explanations provided in the appendix in sections 6.1, 6.2, 6.3, and 6.4.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental Result Reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Sections 3 and 4 have the required information to reproduce the experiments.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item If the paper includes experiments, a No answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and/or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We have shared our code and data in the supplementary. We will be releasing the code publicly before the main conference.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so “No” is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental Setting/Details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Sections 3 and 4 have the required details.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment Statistical Significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Our experiments don't really involve such results that would require error bars or statistical significance tests as they are not distribution-dependent.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The authors should answer "Yes" if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g. negative error rates).
        \item If error bars are reported in tables or plots, The authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments Compute Resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Yes, the GPU used was an A6000 and it took around 7 seconds to get an image generated with its maps. This information is mentioned in section 4.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code Of Ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: It is as per the guidelines.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer No, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader Impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The required discussions are spread across the work. More of it can be found in section 1.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that there is no societal impact of the work performed.
        \item If the authors answer NA or No, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Our model doesn't pose such risks.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The assets used are properly cited and credited.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New Assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The shared data and code is described along with itself.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset/code/model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and Research with Human Subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: No crowdsourcing done.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional Review Board (IRB) Approvals or Equivalent for Research with Human Subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: No such experiments or participants involved.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\end{enumerate}


==> text_fig/text_PID_info.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=5cm]{images/Venn_diagram.png}
    % \includegraphics[width=0.8\linewidth]{images/PID.pdf}
    % % \includegraphics{images/PID.pdf}
    \caption{Partial Information Decomposition (PID) of the I($X_1$,$X_2$;$Y$)}
    \label{fig:venn_diagram}
\end{figure}

==> text_table/text_mIOU.tex <==

\begin{table}[h]
    \centering
    \begin{tabular}{|c|c|}
    \hline
         \textbf{Method} & \textbf{mean IoU} \\
    \hline
         MI & 0.145 \\
    \hline
         CMI & 0.156 \\
    \hline     
         \textbf{PID (Ours)} & \textbf{0.170} \\
    \hline
    \end{tabular}
    \\ 
    \caption{mIoU Scores}
    \label{word_local}
\end{table}
